Positivity conditions on the annulus via the double-layer potential kernel

We introduce and study a scale of operator classes on the annulus that is motivated by the $\mathcal{C}_{\rho}$ classes of $\rho$-contractions of Nagy and Foia\c{s}. In particular, our classes are defined in terms of the contractivity of the double-layer potential integral operator over the annulus. We prove that if, in addition, complete contractivity is assumed, then one obtains a complete characterization involving certain variants of the $\mathcal{C}_{\rho}$ classes. Recent work of Crouzeix-Greenbaum and Schwenninger-de Vries allows us to also obtain relevant K-spectral estimates, generalizing existing results from the literature on the annulus. Finally, we exhibit a special case where these estimates can be significantly strengthened.

==> Bibliography.tex <==
@book {Pick,
    AUTHOR = {Agler, Jim and McCarthy, John E.},
     TITLE = {Pick interpolation and {H}ilbert function spaces},
    SERIES = {Graduate Studies in Mathematics},
    VOLUME = {44},
 PUBLISHER = {American Mathematical Society, Providence, RI},
      YEAR = {2002},
      ISBN = {0-8218-2898-3} }
      


@book{NewPick,
author={Agler, Jim and McCarthy, John E. and Young, Nicholas J.},
place={Cambridge}, series={Cambridge Tracts in Mathematics}, title={Operator Analysis: Hilbert Space Methods in Complex Analysis}, publisher={Cambridge University Press}, year={2020}, collection={Cambridge Tracts in Mathematics}}




@article {AndoNishioconvex,
    AUTHOR = {Ando, Tsuyoshi and Nishio, Katsuyoshi},
     TITLE = {Convexity properties of operator radii associated with unitary
              {$\rho $}-dilations},
   JOURNAL = {Michigan Math. J.},
  FJOURNAL = {Michigan Mathematical Journal},
    VOLUME = {20},
      YEAR = {1973},
     PAGES = {303--307},
}


@article {BadeaCassierConstrained,
    AUTHOR = {Badea, C. and Cassier, G.},
     TITLE = {Constrained von {N}eumann inequalities},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {166},
      YEAR = {2002},
    NUMBER = {2},
     PAGES = {260--297},
}
@article {BadCrouzKlajaradii,
    AUTHOR = {Badea, Catalin and Crouzeix, Michel and Klaja, Hubert},
     TITLE = {Spectral sets and operator radii},
   JOURNAL = {Bull. Lond. Math. Soc.},
  FJOURNAL = {Bulletin of the London Mathematical Society},
    VOLUME = {50},
      YEAR = {2018},
    NUMBER = {6},
     PAGES = {986--996},
}
@article {BergStampskewdil,
    AUTHOR = {Berger, C. A. and Stampfli, J. G.},
     TITLE = {Norm relations and skew dilations},
   JOURNAL = {Acta Sci. Math. (Szeged)},
  FJOURNAL = {Acta Universitatis Szegediensis. Acta Scientiarum
              Mathematicarum},
    VOLUME = {28},
      YEAR = {1967},
     PAGES = {191--195},
}
@article {CassierFackContractions,
    AUTHOR = {Cassier, Gilles and Fack, Thierry},
     TITLE = {Contractions in von {N}eumann algebras},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {135},
      YEAR = {1996},
    NUMBER = {2},
     PAGES = {297--338},
}
@article {CassierSuciuSharpened,
    AUTHOR = {Cassier, Gilles and Suciu, Nicolae},
     TITLE = {Sharpened forms of a von {N}eumann inequality for
              {$\rho$}-contractions},
   JOURNAL = {Math. Scand.},
  FJOURNAL = {Mathematica Scandinavica},
    VOLUME = {102},
      YEAR = {2008},
    NUMBER = {2},
     PAGES = {265--282},
}
@article {CassierHarnack,
    AUTHOR = {Cassier, Gilles and Benharrat, Mohammed and Belmouhoub,
              Soumia},
     TITLE = {Harnack parts of {$\rho$}-contractions},
   JOURNAL = {J. Operator Theory},
  FJOURNAL = {Journal of Operator Theory},
    VOLUME = {80},
      YEAR = {2018},
    NUMBER = {2},
     PAGES = {453--480},
}
@article {Davisshell,
    AUTHOR = {Davis, Chandler},
     TITLE = {The shell of a {H}ilbert-space operator},
   JOURNAL = {Acta Sci. Math. (Szeged)},
  FJOURNAL = {Acta Universitatis Szegediensis. Acta Scientiarum
              Mathematicarum},
    VOLUME = {29},
      YEAR = {1968},
     PAGES = {69--86},
}
@article {DritschelScott,
    AUTHOR = {Dritschel, Michael A. and McCullough, Scott and Woerdeman,
              Hugo J.},
     TITLE = {Model theory for {$\rho$}-contractions, {$\rho\le2$}},
   JOURNAL = {J. Operator Theory},
  FJOURNAL = {Journal of Operator Theory},
    VOLUME = {41},
      YEAR = {1999},
    NUMBER = {2},
     PAGES = {321--350},
}
@article {Durszton,
    AUTHOR = {Durszt, E.},
     TITLE = {On unitary {$\rho $}-dilations of operators},
   JOURNAL = {Acta Sci. Math. (Szeged)},
  FJOURNAL = {Acta Universitatis Szegediensis. Acta Scientiarum
              Mathematicarum},
    VOLUME = {27},
      YEAR = {1966},
     PAGES = {247--250},
}
@article {Dursztfactor,
    AUTHOR = {Durszt, E.},
     TITLE = {Factorization of operators in {$\scr C\sb{\rho }$} classes},
   JOURNAL = {Acta Sci. Math. (Szeged)},
  FJOURNAL = {Acta Universitatis Szegediensis. Acta Scientiarum
              Mathematicarum},
    VOLUME = {37},
      YEAR = {1975},
    NUMBER = {3-4},
     PAGES = {195--199},
     }
@article {Holbrookonthe,
    AUTHOR = {Holbrook, John A. R.},
     TITLE = {On the power-bounded operators of {S}z.-{N}agy and {F}oia\c{s}},
   JOURNAL = {Acta Sci. Math. (Szeged)},
  FJOURNAL = {Acta Universitatis Szegediensis. Acta Scientiarum
              Mathematicarum},
    VOLUME = {29},
      YEAR = {1968},
     PAGES = {299--310},
}
@article {OkuboAndoproducts,
    AUTHOR = {Okubo, K. and Ando, T.},
     TITLE = {Operator radii of commuting products},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {56},
      YEAR = {1976},
     PAGES = {203--210},
      ISSN = {0002-9939},
}
@article {OkuboAndroconstantsrelated,
    AUTHOR = {Okubo, Kazuyoshi and Ando, Tsuyoshi},
     TITLE = {Constants related to operators of class {$C\sb{\rho }$}},
   JOURNAL = {Manuscripta Math.},
  FJOURNAL = {Manuscripta Mathematica},
    VOLUME = {16},
      YEAR = {1975},
    NUMBER = {4},
     PAGES = {385--394},
      ISSN = {0025-2611},
}
@article {OkuboSpitkovsky2x2,
    AUTHOR = {Okubo, Kazuyoshi and Spitkovsky, Ilya},
     TITLE = {On the characterization of {$2\times 2$} {$\rho$}-contraction
              matrices},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {325},
      YEAR = {2001},
    NUMBER = {1-3},
     PAGES = {177--189},
}
@article {PagaczbetweenvonNeumann,
    AUTHOR = {Pagacz, Patryk and Pietrzycki, Pawe\l  and Wojtylak, Micha\l },
     TITLE = {Between the von {N}eumann inequality and the {C}rouzeix
              conjecture},
   JOURNAL = {Linear Algebra Appl.},
  FJOURNAL = {Linear Algebra and its Applications},
    VOLUME = {605},
      YEAR = {2020},
     PAGES = {130--157},
      ISSN = {0024-3795},
}

@article {NagyFoiasoncertainclasses,
    AUTHOR = {Sz.-Nagy, B\'{e}la and Foia\c{s}, Ciprian},
     TITLE = {On certain classes of power-bounded operators in {H}ilbert
              space},
   JOURNAL = {Acta Sci. Math. (Szeged)},
  FJOURNAL = {Acta Universitatis Szegediensis. Acta Scientiarum
              Mathematicarum},
    VOLUME = {27},
      YEAR = {1966},
     PAGES = {17--25},
}
@book {NagyFoiasbook,
    AUTHOR = {Sz.-Nagy, B\'{e}la and Foias, Ciprian and Bercovici, Hari and
              K\'{e}rchy, L\'{a}szl\'{o}},
     TITLE = {Harmonic analysis of operators on {H}ilbert space},
    SERIES = {Universitext},
   EDITION = {Second},
   EDITION = {enlarged},
 PUBLISHER = {Springer, New York},
      YEAR = {2010},
     PAGES = {xiv+474},
      ISBN = {978-1-4419-6093-1},
}
@article {Tsikvonneumann,
    AUTHOR = {Tsikalas, Georgios},
     TITLE = {A von {N}eumann type inequality for an annulus},
   JOURNAL = {J. Math. Anal. Appl.},
  FJOURNAL = {Journal of Mathematical Analysis and Applications},
    VOLUME = {506},
      YEAR = {2022},
    NUMBER = {2},
     PAGES = {Paper No. 125714, 12},
}
@article {WilliamsSchwarz,
    AUTHOR = {Williams, James P.},
     TITLE = {Schwarz norms for operators},
   JOURNAL = {Pacific J. Math.},
  FJOURNAL = {Pacific Journal of Mathematics},
    VOLUME = {24},
      YEAR = {1968},
     PAGES = {181--188},
}
@article {NagyFrench,
    AUTHOR = {Sz.-Nagy, B\'{e}la},
     TITLE = {Sur les contractions de l'espace de {H}ilbert},
   JOURNAL = {Acta Sci. Math. (Szeged)},
  FJOURNAL = {Acta Universitatis Szegediensis. Acta Scientiarum
              Mathematicarum},
    VOLUME = {15},
      YEAR = {1953},
     PAGES = {87--92},
}
@article {Bergerstampflimapping,
    AUTHOR = {Berger, C. A. and Stampfli, J. G.},
     TITLE = {Mapping theorems for the numerical range},
   JOURNAL = {Amer. J. Math.},
  FJOURNAL = {American Journal of Mathematics},
    VOLUME = {89},
      YEAR = {1967},
     PAGES = {1047--1055},
}
@book {Bergerthesis,
    AUTHOR = {Berger, Charles Arnold},
     TITLE = {N{ORMAL} {DILATIONS}},
      NOTE = {Thesis (Ph.D.)--Cornell University},
 PUBLISHER = {ProQuest LLC, Ann Arbor, MI},
      YEAR = {1963},
     PAGES = {67}, 
}
@misc{schwendevries,
  url = {https://arxiv.org/abs/2302.05389},
  author = {Schwenninger, Felix L. and de Vries, Jens},
  title = {On Abstract Spectral Constants},
  publisher = {arXiv},
  year = {2023},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article {Putsand,
    AUTHOR = {Putinar, Mihai and Sandberg, Sebastian},
     TITLE = {A skew normal dilation on the numerical range of an operator},
   JOURNAL = {Math. Ann.},
  FJOURNAL = {Mathematische Annalen},
    VOLUME = {331},
      YEAR = {2005},
    NUMBER = {2},
     PAGES = {345--357},
}






@misc{RansfordOster,
  url = {https://arxiv.org/abs/2011.10422},
  author = {Clouâtre, Raphaël and Ostermann, Maëva and Ransford, Thomas},
  title = {An abstract approach to the Crouzeix conjecture},
  publisher = {arXiv},
  year = {2020},
  copyright = {Creative Commons Attribution 4.0 International}
}
@article {LiCaldwellGreen,
    AUTHOR = {Caldwell, Trevor and Greenbaum, Anne and Li, Kenan},
     TITLE = {Some extensions of the {C}rouzeix-{P}alencia result},
   JOURNAL = {SIAM J. Matrix Anal. Appl.},
  FJOURNAL = {SIAM Journal on Matrix Analysis and Applications},
    VOLUME = {39},
      YEAR = {2018},
    NUMBER = {2},
     PAGES = {769--780},
}
@article {CrouzPal,
    AUTHOR = {Crouzeix, M. and Palencia, C.},
     TITLE = {The numerical range is a {$(1+\sqrt{2})$}-spectral set},
   JOURNAL = {SIAM J. Matrix Anal. Appl.},
  FJOURNAL = {SIAM Journal on Matrix Analysis and Applications},
    VOLUME = {38},
      YEAR = {2017},
    NUMBER = {2},
     PAGES = {649--655},
}
@article {CrouxNumerangeandfunctional,
    AUTHOR = {Crouzeix, Michel},
     TITLE = {Numerical range and functional calculus in {H}ilbert space},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {244},
      YEAR = {2007},
    NUMBER = {2},
     PAGES = {668--690},
}
@article {Delyon,
    AUTHOR = {Delyon, Bernard and Delyon, Fran\c{c}ois},
     TITLE = {Generalization of von {N}eumann's spectral sets and integral
              representation of operators},
   JOURNAL = {Bull. Soc. Math. France},
  FJOURNAL = {Bulletin de la Soci\'{e}t\'{e} Math\'{e}matique de France},
    VOLUME = {127},
      YEAR = {1999},
    NUMBER = {1},
     PAGES = {25--41},
}
@article {RansfordSchwenninger,
    AUTHOR = {Ransford, Thomas and Schwenninger, Felix L.},
     TITLE = {Remarks on the {C}rouzeix-{P}alencia proof that the numerical
              range is a {$(1+\sqrt2)$}-spectral set},
   JOURNAL = {SIAM J. Matrix Anal. Appl.},
  FJOURNAL = {SIAM Journal on Matrix Analysis and Applications},
    VOLUME = {39},
      YEAR = {2018},
    NUMBER = {1},
     PAGES = {342--345},
}
@article {Boundsforanalytical,
    AUTHOR = {Crouzeix, Michel},
     TITLE = {Bounds for analytical functions of matrices},
   JOURNAL = {Integral Equations Operator Theory},
  FJOURNAL = {Integral Equations and Operator Theory},
    VOLUME = {48},
      YEAR = {2004},
    NUMBER = {4},
     PAGES = {461--477},
}
@article {CrouzGreen,
    AUTHOR = {Crouzeix, Michel and Greenbaum, Anne},
     TITLE = {Spectral sets: numerical range and beyond},
   JOURNAL = {SIAM J. Matrix Anal. Appl.},
  FJOURNAL = {SIAM Journal on Matrix Analysis and Applications},
    VOLUME = {40},
      YEAR = {2019},
    NUMBER = {3},
     PAGES = {1087--1101},
}
@article {Tsiknote,
    AUTHOR = {Tsikalas, Georgios},
     TITLE = {A note on a spectral constant associated with an annulus},
   JOURNAL = {Oper. Matrices},
  FJOURNAL = {Operators and Matrices},
    VOLUME = {16},
      YEAR = {2022},
    NUMBER = {1},
     PAGES = {95--99},
}
@misc{belloyak,
  
  url = {https://arxiv.org/abs/2106.08757},
  
  author = {Bello, Glenier and Yakubovich, Dmitry},

  title = {An operator model in the annulus},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}


@article {mcculloughpascoe,
    AUTHOR = {McCullough, Scott and Pascoe, James E.},
     TITLE = {Geometric dilations and operator annuli},
   JOURNAL = {J. Funct. Anal.},
  FJOURNAL = {Journal of Functional Analysis},
    VOLUME = {285},
      YEAR = {2023},
    NUMBER = {7},
     PAGES = {Paper No. 110035}
}




@article {WA,
    AUTHOR = {Suen, Ching-Yun},
     TITLE = {{$W_A$} contractions},
   JOURNAL = {Positivity},
  FJOURNAL = {Positivity. An International Journal devoted to the Theory and
              Applications of Positivity in Analysis},
    VOLUME = {2},
      YEAR = {1998},
    NUMBER = {4},
     PAGES = {301--310},
}
@article {ScottChien,
    AUTHOR = {McCullough, Scott and Shen, Li-Chien},
     TITLE = {On the {S}zeg\H{o} kernel of an annulus},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {121},
      YEAR = {1994},
    NUMBER = {4},
     PAGES = {1111--1121},
}
@book {Paulsenbook,
    AUTHOR = {Paulsen, Vern},
     TITLE = {Completely bounded maps and operator algebras},
    SERIES = {Cambridge Studies in Advanced Mathematics},
    VOLUME = {78},
 PUBLISHER = {Cambridge University Press, Cambridge},
      YEAR = {2002},
     PAGES = {xii+300},
}
@book {Halmosproblembook,
    AUTHOR = {Halmos, Paul Richard},
     TITLE = {A {H}ilbert space problem book},
    SERIES = {Encyclopedia of Mathematics and its Applications},
    VOLUME = {17},
   EDITION = {Second},
 PUBLISHER = {Springer-Verlag, New York-Berlin},
      YEAR = {1982},
     PAGES = {xvii+369},
}
@book {Conway,
    AUTHOR = {Conway, John B.},
     TITLE = {A course in functional analysis},
    SERIES = {Graduate Texts in Mathematics},
    VOLUME = {96},
   EDITION = {Second},
 PUBLISHER = {Springer-Verlag, New York},
      YEAR = {1990},
     PAGES = {xvi+399},
}
@misc{bivariate,
  
  url = {https://arxiv.org/abs/2007.09784},
  
  author = {Crouzeix, Michel and Kressner, Daniel},
  
  keywords = {Functional Analysis (math.FA), Numerical Analysis (math.NA), FOS: Mathematics, FOS: Mathematics, 15A60, 15A16, 65F60},
  
  title = {A bivariate extension of the Crouzeix-Palencia result with an application to Fréchet derivatives of matrix functions},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}
@article {Annuluskspectral,
    AUTHOR = {Crouzeix, Michel},
     TITLE = {The annulus as a {$K$}-spectral set},
   JOURNAL = {Commun. Pure Appl. Anal.},
  FJOURNAL = {Communications on Pure and Applied Analysis},
    VOLUME = {11},
      YEAR = {2012},
    NUMBER = {6},
     PAGES = {2291--2303},
}
@article {Mccshen,
    AUTHOR = {McCullough, Scott and Shen, Li-Chien},
     TITLE = {On the {S}zeg\H{o} kernel of an annulus},
   JOURNAL = {Proc. Amer. Math. Soc.},
  FJOURNAL = {Proceedings of the American Mathematical Society},
    VOLUME = {121},
      YEAR = {1994},
    NUMBER = {4},
     PAGES = {1111--1121},
}
@incollection {badeaspectral,
    AUTHOR = {Catalin Badea and Bernhard Beckermann},
     TITLE = {Spectral Sets},
   EDITION = {\textit{Handbook of Linear Algebra}, (L. Hogben, ed.), second edition},
 PUBLISHER = {CRC Press},
      YEAR = {2013},
}
@article {Harnackcrho,
    AUTHOR = {Cassier, Gilles and Benharrat, Mohammed and Belmouhoub,
              Soumia},
     TITLE = {Harnack parts of {$\rho$}-contractions},
   JOURNAL = {J. Operator Theory},
  FJOURNAL = {Journal of Operator Theory},
    VOLUME = {80},
      YEAR = {2018},
    NUMBER = {2},
     PAGES = {453--480},
     
}
@article {manyauthorscrouz,
    AUTHOR = {Bickel, Kelly and Gorkin, Pamela and Greenbaum, Anne and
              Ransford, Thomas and Schwenninger, Felix L. and Wegert, Elias},
     TITLE = {Crouzeix's conjecture and related problems},
   JOURNAL = {Comput. Methods Funct. Theory},
  FJOURNAL = {Computational Methods and Function Theory},
    VOLUME = {20},
      YEAR = {2020},
    NUMBER = {3-4},
}
@article {Williams,
    AUTHOR = {Williams, James P.},
     TITLE = {Schwarz norms for operators},
   JOURNAL = {Pacific J. Math.},
  FJOURNAL = {Pacific Journal of Mathematics},
    VOLUME = {24},
      YEAR = {1968},
     PAGES = {181--188},
}

@article {Boundsforanalytical,
    AUTHOR = {Crouzeix, Michel},
     TITLE = {Bounds for analytical functions of matrices},
   JOURNAL = {Integral Equations Operator Theory},
  FJOURNAL = {Integral Equations and Operator Theory},
    VOLUME = {48},
      YEAR = {2004},
    NUMBER = {4},
     PAGES = {461--477},
}

@article {Annulusquotients,
    AUTHOR = {McCullough, Scott},
     TITLE = {Isometric representations of some quotients of {$H^\infty$} of
              an annulus},
   JOURNAL = {Integral Equations Operator Theory},
  FJOURNAL = {Integral Equations and Operator Theory},
    VOLUME = {39},
      YEAR = {2001},
    NUMBER = {3},
     PAGES = {335--362},
}














